A Grid-based Method for Removing Overlaps of Dimensionality Reduction Scatterplot Layouts

Dimensionality Reduction (DR) scatterplot layouts have become a ubiquitous visualization tool for analyzing multidimensional datasets. Despite their popularity, such scatterplots suffer from occlusion, especially when informative glyphs are used to represent data instances, potentially obfuscating critical information for the analysis under execution. Different strategies have been devised to address this issue, either producing overlap-free layouts that lack the powerful capabilities of contemporary DR techniques in uncovering interesting data patterns or eliminating overlaps as a post-processing strategy. Despite the good results of post-processing techniques, most of the best methods typically expand or distort the scatterplot area, thus reducing glyphs' size (sometimes) to unreadable dimensions, defeating the purpose of removing overlaps. This paper presents Distance Grid (DGrid), a novel post-processing strategy to remove overlaps from DR layouts that faithfully preserves the original layout's characteristics and bounds the minimum glyph sizes. We show that DGrid surpasses the state-of-the-art in overlap removal (through an extensive comparative evaluation considering multiple different metrics) while also being one of the fastest techniques, especially for large datasets. A user study with 51 participants also shows that DGrid is consistently ranked among the top techniques for preserving the original scatterplots' visual characteristics and the aesthetics of the final results.

==> use_case_images.tex <==
% \section{Exploring image dataset}
\noindent\paragraph{Image dataset.}

In this use case, we explore an image dataset using the features generated after training a Convolutional Neural Network (CNN). Our architecture has two convolutional layers, followed by a dense layer with 128 neurons, followed by a softmax layer with 10 neurons. We randomly selected $3000$ images from the Fashion MNIST~\cite{Xiao2017} dataset and used the dense layer as features. Fig.~\ref{fig:image-analysis}(A) shows a UMAP~\cite{mcinnes2020umap} projection of the dataset. The circles' colors give us information about which classes are similar to one another. However, to understand what the CNN learned during the training process, it is interesting to investigate the images associated with each data sample.


\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/results/usecases/image-analysis}
    \caption{Using DGrid to get a better view of image exploration. To understand CNN learned features, we project a subset of samples (A). Then, we select a cluster of interest to investigate the similarity between data samples (B), which cannot be performed due to overlap. After running DGrid on the selected cluster (C) and visualizing explanations (D), it is possible to understand the importance of CNN to each part of the images.}
    \label{fig:image-analysis}
\end{figure*}

Fig.~\ref{fig:image-analysis}(B) shows how drawing the images of each data sample would look without overlap removal. There is no way to perform intra-cluster analysis or understand why a few data samples from other classes were projected together with the purple one. Running DGrid on the images (C) helps us to visualize the structures inside the cluster and how CNN learned the features to separate purples with visible handles (left side) and purses without visible handles (right side).

Finally, the images with borders were misclassified by the CNN, and the colors indicate the correct class. While we expect that the CNN has confused those images with purses, we use SHAP~\cite{Lundberg2017} to explain which part of the images contributes to the confusion. Fig.~\ref{fig:image-analysis}(D) shows the contribution of each part of the image to increase (in red) or to decrease (in blue) the probability of every class. Notice the selected image was misclassified as a purse due to the format and color intensity of the dress (see the SHAP values for the image inside the dashed square). For instance, the top part of the dress was probably misunderstood as a handle. This fact is testified by the explanations of neighborhood images, in which the rectangular shape and visible handles contribute to augmenting the probability of that class. 

